LLaMA-Omni: Seamless Speech Interaction with Large Language Models

Models like GPT-4o enable real-time interaction with large language models (LLMs) through speech, significantly enhancing user experience compared to traditional text-based interaction. However, there is still a lack of exploration on how to build speech interaction models based on open-source LLMs. To address this, we propose LLaMA-Omni, a novel model architecture designed for low-latency and high-quality speech interaction with LLMs. LLaMA-Omni integrates a pretrained speech encoder, a speech adaptor, an LLM, and a streaming speech decoder. It eliminates the need for speech transcription, and can simultaneously generate text and speech responses directly from speech instructions with extremely low latency. We build our model based on the latest Llama-3.1-8B-Instruct model. To align the model with speech interaction scenarios, we construct a dataset named InstructS2S-200K, which includes 200K speech instructions and corresponding speech responses. Experimental results show that compared to previous speech-language models, LLaMA-Omni provides better responses in both content and style, with a response latency as low as 226ms. Additionally, training LLaMA-Omni takes less than 3 days on just 4 GPUs, paving the way for the efficient development of speech-language models in the future.

==> Figures/figure_prompt.tex <==
\begin{figure}[t]
\small
\begin{tcolorbox}[colback=blue!10,colframe=blue!50!black,arc=1mm,boxrule=1pt,left=1mm,right=1mm,top=1mm,bottom=1mm]

\begin{verbatim}
<|begin_of_text|><|start_header_id|>system<|end_header_id|>

You are a helpful language and speech assistant. You are able to
understand the speech content that the user provides, and assist the 
user with a variety of tasks using natural language.<|eot_id|>
<|start_header_id|>user<|end_header_id|>
\end{verbatim}
\texttt{\textbf{<speech>}}
\begin{verbatim}
Please answer the questions in the user's input speech.<|eot_id|>
<|start_header_id|>assistant<|end_header_id|>
\end{verbatim}

\end{tcolorbox}
\caption{Prompt template of \name.}
\label{fig:prompt}
\end{figure}


==> Figures/figure_training.tex <==
% \begin{wrapfigure}{R}{0.5\linewidth}
    % \vspace{-10pt}
\begin{figure}
    \centering
    \includegraphics[width=0.6\linewidth]{Figures/training.pdf}
    \caption{Illustration of the two-stage training strategy for \name.}
    \label{fig:training}
\end{figure}
    % \vspace{-10pt}
% \end{wrapfigure}

==> Sections/460_decoding_time.tex <==

Table~\ref{tab:time} lists the average decoding times of different models on the S2TIF and S2SIF tasks. For the S2TIF task, SpeechGPT needs to first output the text instruction and then the text response, while SALMONN and Qwen2-Audio tend to produce lengthy responses. In contrast, \name provides concise answers directly, resulting in significantly lower decoding times, with an average of only 1.49 seconds per instruction. For the S2SIF task, SpeechGPT serially outputs the text and speech responses, resulting in a decoding time approximately 6 times longer than when generating only text responses. In contrast, \name outputs both text and speech responses simultaneously and employs a non-autoregressive architecture for generating discrete units. As a result, the total generation time only increases by 1.28 times, demonstrating \name's advantage in decoding speed.

==> Tables/table_decode_time.tex <==

\begin{wraptable}{R}{0.3\linewidth}
% \begin{table}[t]
\vspace{-20pt}
% \centering
\caption{Average decoding time (s) of different models on S2TIF and S2SIF tasks.}
% \vspace{5pt}
\label{tab:time}
\begin{center}
\resizebox{\linewidth}{!}{
\begin{tabular}{lcc}
\toprule
\textbf{Model} & \textbf{S2TIF} & \textbf{S2SIF} \\
\midrule
\textbf{SpeechGPT }    & 4.28  & 25.60 \\
\textbf{SALMONN}       & 4.78  & /     \\
\textbf{Qwen2-Audio}   & 8.42  & /     \\
\textbf{\name}         & \textbf{1.49}  & \textbf{1.92}  \\
\bottomrule
\end{tabular}}
\end{center}
% \end{table}
\end{wraptable}

==> Tables/table_latency.tex <==
\begin{table}[t]
% \centering
\caption{Latency, speech-text alignment and speech quality under different unit chunk sizes.}
\vspace{5pt}
\label{tab:latency}
\begin{center}
\small
% \resizebox{\linewidth}{!}{
\begin{tabular}{ccccccc}
\toprule
\textbf{Chunk Size $\Omega$} & \textbf{Latency (ms)} & \textbf{\#Lagging Word} & \textbf{ASR-WER $\downarrow$} & \textbf{ASR-CER $\downarrow$} & \textbf{UTMOS $\uparrow$} \\
\midrule
10   & \textbf{226.13}  & \textbf{1.82}  & \textbf{10.44} & \textbf{6.94} & 3.2304 \\
20   & 256.28  & 2.83  & 10.51 & 6.98 & 3.4748 \\
40   & 326.63  & 4.68  & 10.99 & 7.24 & 3.6688 \\
60   & 391.96  & 6.47  & 11.17 & 7.27 & 3.7549 \\
80   & 467.34  & 8.29  & 11.40 & 7.45 & 3.7858 \\
100  & 527.64  & 10.02 & 11.48 & 7.45 & 3.8242 \\
$+\infty$   & 1924.62 & 41.40 & 11.61 & 7.59 & \textbf{3.9296} \\
\bottomrule
\end{tabular}
% }
\end{center}
\end{table}
